The Generalized Label Correcting Method for Optimal Kinodynamic Motion Planning

Nearly all autonomous robotic systems use some form of motion planning to compute reference motions through their environment. An increasing use of autonomous robots in a broad range of applications creates a need for efficient, general purpose motion planning algorithms that are applicable in any of these new application domains. This thesis presents a resolution complete optimal kinodynamic motion planning algorithm based on a direct forward search of the set of admissible input signals to a dynamical model. The advantage of this generalized label correcting method is that it does not require a local planning subroutine as in the case of related methods. Preliminary material focuses on new topological properties of the canonical problem formulation that are used to show continuity of the performance objective. These observations are used to derive a generalization of Bellman's principle of optimality in the context of kinodynamic motion planning. A generalized label correcting algorithm is then proposed which leverages these results to prune candidate input signals from the search when their cost is greater than related signals. The second part of this thesis addresses admissible heuristics for kinodynamic motion planning. An admissibility condition is derived that can be used to verify the admissibility of candidate heuristics for a particular problem. This condition also characterizes a convex set of admissible heuristics. A linear program is formulated to obtain a heuristic which is as close to the optimal cost-to-go as possible while remaining admissible. This optimization is justified by showing its solution coincides with the solution to the Hamilton-Jacobi-Bellman equation. Lastly, a sum-of-squares relaxation of this infinite-dimensional linear program is proposed for obtaining provably admissible approximate solutions.

==> appe.tex <==
\chapter{Graph Search Algorithms} 

\bibliographystyle{amsalpha}
\bibliography{appe}

\clearpage
\newpage


==> biblio.tex <==
%% This defines the bibliography file (main.bib) and the bibliography style.
%% If you want to create a bibliography file by hand, change the contents of
%% this file to a `thebibliography' environment.  For more information 
%% see section 4.3 of the LaTeX manual.
\begin{singlespace}
\bibliography{main}
\bibliographystyle{plain}
\end{singlespace}


==> cite/README <==
This directory contains four .sty files that are mutually compatible,
but (mostly) independent:

cite.sty       Compressed, sorted lists of numerical citations: [8,11-16]
               with many options for controlling the formatting.

overcite.sty   like \usepackage[superscript]{cite}

drftcite.sty   Print the tags instead of the numbers for \cite and \bibitem.

chapterbib.sty Do multiple bibliographies--one for each \include file.

The user manuals for cite and chapterbib are LaTeX files cite.ltx
and chapterbib.ltx, and already typeset pdf versions.

They are all released under a very simple permissive license in
the MIT/BSD style:  They may be freely used, transmitted, reproduced, 
or modified provided that the copyright and permission notice is 
left intact.



Donald Arseneau                         asnd@triumf.ca


==> signature.tex <==
% -*- Mode:TeX -*-
%
% Some departments (e.g. Chemistry) require an additional cover page
% with signatures of the thesis committee.  Please check with your
% thesis advisor or other appropriate person to determine if such a 
% page is required for your thesis.  
%
% If you choose not to use the "titlepage" environment, a \newpage
% commands, and several \vspace{\fill} commands may be necessary to
% achieve the required spacing.  The \signature command is defined in
% the "mitthesis" class
%
% The following sample appears courtesy of Ben Kaduk <kaduk@mit.edu> and
% was used in his June 2012 doctoral thesis in Chemistry. 

\begin{titlepage}
\begin{large}
This doctoral thesis has been examined by a Committee of the Department
of Chemistry as follows:

\signature{Professor Domitilla Del Vecchio}{Chair, Thesis Committee \\
   Professor of Mechanical Engineering}

\signature{Professor Emilio Frazzoli}{Thesis Supervisor \\
   Professor of Aerospace and Astronautics}

\signature{Dr. Karl Iagnemma}{Member, Thesis Committee \\
   Principal Research Scientist in the Department of Mechanical Engineering}
\end{large}
\end{titlepage}


